Row-Merged Polar Codes: Analysis, Design and Decoder Implementation

Row-merged polar codes are a family of pre-transformed polar codes (PTPCs) with little precoding overhead. Providing an improved distance spectrum over plain polar codes, they are capable to perform close to the finite-length capacity bounds. However, there is still a lack of efficient design procedures for row-merged polar codes. Using novel weight enumeration algorithms with low computational complexity, we propose a design methodology for row-merged polar codes that directly considers their minimum distance properties. The codes significantly outperform state-of-the-art cyclic redundancy check (CRC)-aided polar codes under successive cancellation list (SCL) decoding in error-correction performance. Furthermore, we present fast simplified successive cancellation list (Fast-SSCL) decoding of PTPCs, based on which we derive a high-throughput, unrolled architecture template for fully pipelined decoders. Implementation results of SCL decoders for row-merged polar codes in a 12 nm technology additionally demonstrate the superiority of these codes with respect to the implementation costs, compared to state-of-the-art reference decoder implementations.

==> figures/register.tex <==
\usepackage{pgf,tikz}
\usepackage{pgfplots}
\usetikzlibrary{calc}
\usepackage{amsmath}

\makeatletter

\pgfdeclareshape{reg}{
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.325\pgf@x
    \pgf@y=0.325\pgf@y
  }
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.325\pgf@x
    \pgf@y=-0.325\pgf@y
  }
  \inheritanchorborder[from=rectangle]

  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{\northeast}
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  \anchor{D}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.5\pgf@y%
  }
  \anchor{CLK}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.66666\pgf@y%
  }
  \anchor{Q}{
    \pgf@process{\northeast}%
    \pgf@y=.5\pgf@y%
  }
  \backgroundpath{
    \pgfpathrectanglecorners{\southwest}{\northeast}
    \pgf@anchor@reg@CLK
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgf@xc=\pgf@x \pgf@yc=\pgf@y
    \pgfmathsetlength\pgf@x{0.5ex} %
    \advance\pgf@ya by \pgf@x
    \advance\pgf@xb by \pgf@x
    \advance\pgf@yc by -\pgf@x
    \pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
    \pgfclosepath

  }
}

\tikzset{add font/.code={\expandafter\def\expandafter\tikz@textfont\expandafter{\tikz@textfont#1}}} 

\tikzset{flip flop/port labels/.style={font=\sffamily\scriptsize}}
\tikzset{every reg node/.style={draw,minimum width=1.0cm,minimum height=1.6cm,thick,inner sep=1mm,outer sep=0pt,cap=round}}  %

\makeatother


==> sec_weight_enum.tex <==
\section{Counting Minimum Weight Codewords of Pre-Transformed Polar Codes}\label{sec:counting}

Our goal is to find the minimum distance $\dmin$ and the corresponding number of $\dmin$-weight codewords $\Admin$ of a \ac{PTPC} $\C$.
For this, we will exploit the underlying structure of polar codes. 
Thus, our method is best suited for \acp{PTPC} $\C$ with polar-like rate-profile~$\mathcal I$ and upper-triangular pre-transformation matrix~$\boldsymbol{T}$.
To simplify the problem, the general approach is to split the code $\C = \{\boldsymbol{0}\} \cup \bigcup_{i \in \mathcal I} \Ci$ into $K=|\mathcal I|$ distinct \emph{cosets} ${\Ci = \left\{\boldsymbol{u} \cdot \boldsymbol{G}_N \,\middle|\, \boldsymbol{u} \in \Qi\right\}}$ which 
are obtained by the one-to-one polar transform mapping $\boldsymbol{G}_N$ of the pre-transformed messages
\begin{equation}\label{eq:coset messages}
    \Qi = \left\{\boldsymbol{t}_i \oplus \bigoplus_{h \in \mathcal{H}} \boldsymbol{t}_h\,\middle|\,\mathcal{H} \subseteq \mathcal{I} \setminus \mathbb{Z}_{i+1} \right\}.
\end{equation}
In other words, $\Ci$ contains all codewords whose corresponding messages $\Qi$ have their first non-zero bit in position $i$. 
The row $\boldsymbol{g}_i$ is called the \emph{coset leader} of $\Ci$.
Instead of examining the whole code at once, each coset can be considered individually.
We subsequently denote \emph{plain} (i.e., without pre-transform) and \emph{universal} (i.e., without considering a specific rate-profile) polar cosets by ${\mathcal{P}_i(\mathcal I) = \mathcal{P}_i(\mathcal{I},\boldsymbol{T}=\boldsymbol{I}_N)}$ and $\mathcal{P}_i=\mathcal{P}_i(\mathcal I=\mathbb{Z}_N)$, respectively.
Their corresponding messages are denoted by $\mathcal{Q}_i(\mathcal{I}) = \mathcal{Q}_i(\mathcal{I},\boldsymbol{I}_N)$ and $\mathcal{Q}_i=\mathcal{Q}_i(\mathbb{Z}_N)$.


\subsection{Minimum Distance of \acp{PTPC}}
To find the number of $\dmin$-weight codewords, the minimum distance must be considered first.
For this, we review a lower bound on the minimum distance $\dmin(\C)$ of a \ac{PTPC}.
As shown in \cite{RowshanFormation}, any codeword in a universal coset $\mathcal P_i$ has at least the Hamming weight of the coset leader $\boldsymbol{g}_i$, i.e.,
\begin{equation}\label{eq:UTPdmin}
    \w\left(\boldsymbol{g}_i \oplus \bigoplus\limits_{h \in \mathcal{H}} \boldsymbol{g}_h\right) \geq \w(\boldsymbol{g}_i) = w_i,
\end{equation}
for all $\mathcal H \subseteq \mathbb Z_{i+1:N}$.
From $\mathcal{P}_i(\mathcal{I}) \subseteq \mathcal{P}_i$ and $\boldsymbol{g}_i \in \mathcal{P}_i(\mathcal{I})$ follows that the minimum weight of the codewords of $\mathcal{P}_i(\mathcal{I})$ is $\w(\boldsymbol{g}_i)$.
The Hamming weight of a row $\boldsymbol g_i$ can be efficiently calculated as ${\w(\boldsymbol g_i)=2^{\w(i)}}$ \cite{RowshanFormation}.
Consequently, the minimum distance of a plain polar code $\mathcal{P}(\mathcal{I})$ is found as 
\begin{equation*}
    \dmin(\mathcal{P}(\mathcal{I}))=\min_{i \in \mathcal{I}}\left\{\boldsymbol{g}_i\right\}=\min_{i \in \mathcal{I}}\left\{2^{\w(i)}\right\}.
\end{equation*}
For an upper-triangular pre-transformation matrix $\boldsymbol{T}$ follows $\Ci \subseteq \mathcal{P}_i(\mathcal{I}) \subseteq \mathcal{P}_i$.
Therefore, we find with Eq.~(\ref{eq:UTPdmin}) that the codewords of $\Ci$ have at least the Hamming weight $\w(\boldsymbol{g}_i)$ of the coset leader $\boldsymbol{g}_i$.
Hence, a lower bound on the minimum distance of \acp{PTPC} can be derived as
\begin{equation}\label{eq:dmin lower bound}
    \dmin(\C) \geq \dmin(\mathcal{P}(\mathcal{I})) = \wmin.
\end{equation}
In the following, the lowest potential codeword weight ${\wmin=\wmin(\mathcal{I})}$ is a constant dependent only on the (fixed) rate-profile $\mathcal{I}$ of the given \ac{PTPC} $\C$.

\subsection{Minimum Weight Codewords of \acp{PTPC}}
Following the lower bound in Eq.~(\ref{eq:dmin lower bound}), two cases occur for the minimum distance $\dmin$ of a \ac{PTPC} $\C$:
\begin{enumerate}
    \item $\dmin(\C) = \wmin$: \newline
    The minimum distance is equal to the lower bound and thus $\Awmin(\C) > 0$.
    We consider this case and propose an enumeration method that counts the codewords with weight $\wmin$ of a \ac{PTPC} $\C$.
    
    \item $\dmin(\C) > \wmin$: \newline
    The minimum distance is greater than the lower bound, as all $\wmin$-weight codewords have been eliminated by the pre-transform $\boldsymbol{T}$.
    In this case, the proposed algorithm will just find $\Awmin(\C) = 0$.
    Consequently, more general methods as introduced in \cite{Miloslavskaya2022partialweightdistribution} or \cite{PartialEnumPAC} have to be applied to find $\dmin$ and $\Admin$ of $\C$.
\end{enumerate}

Our method is based on the construction of $\wmin$-weight codewords of polar codes introduced in \cite{RowshanFormation}.
Following this formalism, the enumeration algorithm proposed in \cite{Rowshan2023Impact} counts the codewords of weight $\wmin$ of \ac{PAC} codes.
We will generalize this method to arbitrary \acp{PTPC} and reduce the complexity by eliminating all redundant operations.
From ${\Ci \subseteq \mathcal{P}_i}$ and Eq.~(\ref{eq:UTPdmin}) follows that only cosets with coset index 
\begin{equation*}
    i \in \mathcal{I}_{\wmin} = \left\{j \in \mathcal{I} \,\middle|\, \w(\boldsymbol{g}_j) = \wmin\right\}
\end{equation*}
can contain codewords of weight $\wmin$.
Hence, only these cosets or the respective message sets which generate them have to be considered for the computation of $A_{\wmin}(\C)$.
The set of (pre-transformed) messages that form the $\wmin$-weight codewords $\mathcal{P}_{i,\wmin}(\mathcal{I},\boldsymbol{T})$ of a coset $\Ci$ are defined as
\begin{equation*}
    \mathcal{Q}_{i,\wmin}(\mathcal{I},\boldsymbol{T}) = \left\{\boldsymbol{u} \in \Qi \,\middle|\, \w(\boldsymbol{u} \cdot \boldsymbol{G}_N) = \wmin \right\}.
\end{equation*}
Consequently, 
the number of $\wmin$-weight codewords of a \ac{PTPC} can be found as 
\begin{equation}\label{eq:Awmin}
    A_{\wmin}(\C) = \sum_{i \in \mathcal{I}_{\wmin}} \left|\mathcal{Q}_{i,\wmin}(\mathcal{I},\boldsymbol{T})\right|.
\end{equation}
The formalism introduced in \cite{RowshanFormation} allows to find all messages ${\mathcal{Q}_{i,\wmin} = \mathcal{Q}_{i,\wmin}(\mathbb{Z}_N,\boldsymbol{I}_N)}$ that form the codewords with weight $\wmin=\w(\boldsymbol{g}_i)$ of a universal polar coset $\mathcal{P}_i$.
Since both $\mathcal{Q}_{i,\wmin} \subseteq \mathcal{Q}_i$ and $\Qi \subseteq \mathcal{Q}_i$, we can find the messages that generate the $\wmin$-weight codewords of a polar coset $\Ci$ by the intersection of the two considered message sets as
\begin{equation*}
    \mathcal{Q}_{i,\wmin}(\mathcal{I},\boldsymbol{T}) =  \Qi \cap \mathcal{Q}_{i,\wmin}.
\end{equation*}
The set of ``1'' bit positions $\operatorname{supp}(\boldsymbol{u})$ of a message $\boldsymbol{u}$ directly corresponds to the row combination $\boldsymbol{u} \cdot \boldsymbol{G}_N = \bigoplus_{h \in \operatorname{supp}(\boldsymbol{u})} \boldsymbol{g}_h$.
The construction of codewords of a universal polar coset $\mathcal{P}_i$ with weight 
\begin{equation}
    \w(\boldsymbol{u} \cdot \boldsymbol{G}_N) = \w\left(\vphantom{\bigoplus\limits_{m \in \mathcal{M}_i(\mathcal{J})} \boldsymbol g_m}\right. \underbrace{\boldsymbol{g}_i}_{\substack{\text{coset}\\\text{leader}}} \oplus \underbrace{\bigoplus\limits_{j \in \mathcal{J}} \boldsymbol{g}_j}_\text{core rows} \oplus \underbrace{\bigoplus\limits_{m \in \mathcal{M}_i(\mathcal{J})} \boldsymbol{g}_m}_\text{balancing rows}\,\left.\vphantom{\bigoplus\limits_{m \in \mathcal{M}_i(\mathcal{J})} \boldsymbol{g}_m}\right) = \w(\boldsymbol{g}_i)
\end{equation}
can be formulated by the combination of the coset leader $\boldsymbol{g}_i$ with a set of \emph{core rows} $\mathcal{J} \subseteq \mathcal{K}_i$ and dependent \emph{balancing rows} $\mathcal{M}_i(\mathcal{J}) \subseteq \mathcal{K}_i^\mathrm{c}$.
Thus, the set of ``1'' bit positions of a message $\boldsymbol{u}$ that forms a codeword of weight $\wmin=\w(\boldsymbol{g}_i)$ of $\mathcal{P}_i$ is 
\begin{equation}\label{eq:Ui set}
    \operatorname{supp}(\boldsymbol{u}(i,\mathcal{J})) = \mathcal{U}_i(\mathcal{J}) = \{i\} \cup \mathcal{J} \cup \mathcal{M}_i(\mathcal{J}).
\end{equation}
Hence, the set of all messages $\boldsymbol{u}$ that form the $\wmin$-weight codewords of a universal polar coset $\mathcal{P}_i$ is
\begin{equation}\label{eq:Qiwmin}
    \begin{split}
        \mathcal{Q}_{i,\wmin} = \mathcal{Q}_{i,\wmin}(\mathbb{Z}_N,\boldsymbol{I}_N) = \left\{\boldsymbol{u}(i,\mathcal{J})\,\middle|\,\mathcal{J} \subseteq \mathcal{K}_i\right\}.
    \end{split}
\end{equation}
The core rows $\mathcal{J} \subseteq \mathcal{K}_i$ are found as subsets of the (subsequent) rows that individually do not increase the weight of the coset leader $\boldsymbol g_i$ as
\begin{equation}\label{eq:ki}
    \mathcal K_i = \left\{ j \in \mathbb Z_{i+1:N} \,\middle|\, \w(\boldsymbol g_i \oplus \boldsymbol g_j) = \w(\boldsymbol g_i) \right\}.
\end{equation}
The corresponding complementary set is $\mathcal K_i^\mathrm{c} = \mathbb Z_{i+1:N} \setminus \mathcal K_i$.
As shown in \cite{RowshanFormation}, the Hamming weight of the sum of two rows can be computed as 
\begin{equation}\label{eq:merged row weight}
    \w(\boldsymbol g_i \oplus \boldsymbol g_j) = 2^{\w(i)} + 2^{\w(j)} - 2^{\w(i \land j)+1}.
\end{equation}
For $i < j$, $\w(j)-\w(i~\land~j)=\w(\bar i~\land~j)$ is fulfilled.
Thus, with Eq.~(\ref{eq:merged row weight}) we find for $i < j$ that
\begin{equation}\label{eq:cond increase weight}
    \begin{split}
        j \in \mathcal K_i \Leftrightarrow \w(\boldsymbol g_i \oplus \boldsymbol g_j) = \w(\boldsymbol g_i) &\Leftrightarrow \w(\bar i \land j) = 1,\\
        j \in \mathcal K_i^\mathrm{c} \Leftrightarrow \w(\boldsymbol g_i \oplus \boldsymbol g_j) > \w(\boldsymbol g_i) &\Leftrightarrow \w(\bar i \land j) > 1,        
    \end{split}
\end{equation}
efficiently checking if $j \in \mathcal{K}_i$ or $j \in \mathcal{K}_i^\mathrm{c}$.
As each core row-combination $\mathcal{J} \subseteq \mathcal{K}_i$ identifies one $\wmin$-weight codeword, the number of these codewords in $\mathcal {P}_i$ is $\left|\mathcal{Q}_{i,\wmin}\right|= 2^{\left|\mathcal{K}_i\right|}$.

In addition to a set of core rows $\mathcal J \subseteq \mathcal{K}_i^\mathrm{c}$, the balancing rows ${\mathcal M_i(\mathcal J) \subseteq \mathcal K_i^\mathrm{c}}$ are required to obtain a $\wmin$-weight codeword.
Following \cite[Alg.~2]{Rowshan2023Impact}, the balancing row set $\mathcal M_i(\mathcal J)$ can be computed iteratively, starting with $\mathcal M_i(\emptyset) = \emptyset$, as
\begin{equation}\label{eq:Mset}
    \mathcal{M}_i\left(\tilde{\mathcal{J}} \cup \{j\}\right) = \mathcal{M}_i\left(\tilde{\mathcal{J}}\right) \setxor \tilde{\mathcal{M}}_i\left(j,\tilde{\mathcal{J}}\right),
\end{equation}
where $j \in \mathcal{J} \setminus \tilde{\mathcal{J}}$, $\tilde{\mathcal{J}} \subset \mathcal{J}$, and
\begin{equation}\label{eq:add to Mset}
    \tilde{\mathcal{M}}_i(j,\mathcal {J}) = \underset{{\substack{k \in \mathcal{J} \cup \mathcal{M}_i(\mathcal{J}),\\\bar{i} \land j \land k = 0}}}{\bigsetxor} \left\{\mu_i(j,k)\right\}
\end{equation}
with\footnote{The direct translation from \cite{Rowshan2023Impact} into our notation would be ${\mu_i(j,k) = (\bar i \land (j \lor k)) \lor (i \land j \land k)}$, but since ${\bar i \land j \land k = 0}$ implies ${i \land j \land k = j \land k}$, we can simplify the expression.} ${\mu_i(j,k) = (\bar i \land (j \lor k)) \lor (j \land k)}$.
Using this formalism, we can compute all messages $\mathcal{Q}_{i,\wmin}$ that generate a codeword with weight $\wmin=\w(\boldsymbol{g}_i)$ of a universal polar coset $\mathcal{P}_i$.
Thus, the number of $\wmin$-weight codewords of a polar coset $\Ci$ can be found as
\begin{equation}\label{eq:intersection cardinality}
    \left|\mathcal{Q}_{i,\wmin}(\mathcal{I},\boldsymbol{T})\right| = \left|\Qi \cap \mathcal{Q}_{i,\wmin}\right|.
\end{equation}
A na\"ive approach of computing $\left|\mathcal{Q}_{i,\wmin}(\mathcal{I},\boldsymbol{T})\right|$ that involves finding all elements of $\Qi$ or $\mathcal{Q}_{i,\wmin}$ one by one naturally entails a high computational complexity.
In the following, we will propose a low-complexity method to compute Eq.~(\ref{eq:intersection cardinality}).

\subsection{Message Trees}
Our approach is to represent the message sets $\Qi$ and $\mathcal{Q}_{i,\wmin}$ as binary trees and then compute their intersection.

\begin{definition}[\Acf{DBT}]\label{def:dichotomous binary tree}
    \normalfont
    A \ac{DBT} is a binary tree that has, apart from the root node, two distinct types of levels:
    \begin{enumerate}
        \item \emph{Einzelchild levels $\mathcal{L}_1$}: 
        All nodes do not have a sibling. 
        \item \emph{Sibling levels $\mathcal{L}_2$}: 
        All nodes share their parent node with a sibling node.
    \end{enumerate}   
    The value of each node is either ``0'' or ``1'', where a left child node is always ``0'' and a right child node is always ``1''. If all leaf nodes are at the last level, the tree is called a \ac{PDBT}.
\end{definition}

\begin{proposition}\label{proposition:dichotomous binary tree}
    A set of binary vectors $\mathcal{B} \subseteq \mathbb{F}_2^N$ can be represented by the full paths through a \ac{PDBT} of height 
    $N$ if and only if the set has cardinality $\left|\mathcal{B}\right|=2^{\left|\mathcal{L}^*\right|}$, where
    \begin{equation} \label{eq:sibling levels}
        \mathcal{L}^* = \left\{\min\left\{l \in \mathbb{Z}_N \,\middle|\, b_l \neq b_{\smash{l}}'\right\}\,\middle|\,\boldsymbol{b},\boldsymbol{b}' \in \mathcal{B},\, \boldsymbol{b} \neq \boldsymbol{b}'\right\}
    \end{equation}  
    is the set of levels that contain sibling nodes.
\end{proposition}
\begin{proof}
    ``$\Rightarrow$'':
    Any set $\mathcal{B} \subseteq \mathbb{F}_2^N$, where $b_0=b_{\smash{0}}'$ for all ${\boldsymbol{b},\boldsymbol{b}' \in \mathcal{B}}$, can be represented as a binary tree.
    Therefore, from Eq.~(\ref{eq:sibling levels}) directly follows ${\left|\mathcal{B}\right| \leq 2^{\left|\mathcal{L}^*\right|}}$.
    For ${\left|\mathcal{B}\right| < 2^{\left|\mathcal{L}^*\right|}}$, a node at a sibling level $\mathcal{L}^*$ would have no sibling node. 
    Consequently, the set must have cardinality $\left|\mathcal{B}\right|=2^{\left|\mathcal{L}^*\right|}$ for the corresponding binary tree to be dichotomous.
    
    ``$\Leftarrow$'': 
    A \ac{PDBT} has sibling layers $\mathcal{L}_2$ and thus $2^{\left|\mathcal{L}_2\right|}$ leaf nodes.
    Consequently, the analogous set $\mathcal{B}$ of full paths through the tree has cardinality $\left|\mathcal{B}\right|=2^{\left|\mathcal{L}_2\right|}$ and ${\mathcal{L}^*=\mathcal{L}_2}$.
\end{proof}

\begin{figure}[!t]
	\centering
    \begin{subfigure}[b]{0.48\textwidth}
                \resizebox{\columnwidth}{!}%
                {\input{figures/tree_universal}}
                \caption{ \ac{PDBT} of $\mathcal{Q}_{i=10,\wmin=4}$, branching before each bit $u_h$, $h \in \mathcal{K}_{i=4}=\mathcal{L}_2$.\newline
                }
                \label{subfig:tree_universal}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.48\textwidth}
                \resizebox{\columnwidth}{!}%
                {\input{figures/tree_rate_profile}}
                \caption{ \ac{PDBT} of $\mathcal{Q}_{i=10}(\mathcal{I})$, with non-decreasing rate-profile ${\mathcal{I}}$, %
                branching before each bit $u_h$, $h \in \mathcal{I} \setminus \mathbb{Z}_{i+1}=\mathcal{L}_2$.}
                \label{subfig:tree_rate_profile}
        \end{subfigure}
        \vspace{-.2cm}
    \caption{
        Message trees of a universal polar coset (a) and a plain polar coset (b) for $N=16$ and $i=10$. The intersection of the trees (i.e., common messages $\boldsymbol{u}$) is highlighted. In this example, $\left|\mathcal{Q}_{i=10,\wmin=4}(\mathcal{I})\right|=4$.
    }
    \label{fig:weightenumtree}
\end{figure}


\begin{proposition}\label{proposition: Qi tree}
    The message set $\Qi$ corresponding to arbitrary polar coset $\Ci$ can be represented as a \ac{PDBT} with sibling levels ${\mathcal{L}_2 = \mathcal{I} \setminus \mathbb{Z}_{i+1}}$.
\end{proposition}
\begin{proof}
    The individual bits of a pre-transformed message ${\boldsymbol{u} \in \Qi}$ are found as
    \begin{equation}\label{eq:pretransform naive}
        u_k = v_k \oplus t_{i,k} \oplus \bigoplus_{h=i+1}^{k-1} v_h \cdot t_{h,k},\; 
    \end{equation}
    with $v_i=1$, $v_k \in \mathbb{F}_2$ for $k \in \mathcal{I} \setminus \mathbb{Z}_{i+1}$ and $v_k=0$ otherwise.
    This directly implies ${\mathcal{L}_2 = \mathcal{I} \setminus \mathbb{Z}_{i+1}}$ and $\left|\Qi\right|=2^{\left|\mathcal{I} \setminus \mathbb{Z}_{i+1}\right|}$.
    Thus, per Prop.~\ref{proposition:dichotomous binary tree}, $\Qi$ can be represented as a \ac{PDBT}.
\end{proof}
Following Prop.~\ref{proposition: Qi tree}, a tree-based approach can be used to efficiently compute the messages $\boldsymbol{u} \in \Qi$.
The complexity of finding the pre-transformed messages $\boldsymbol{u}$ from messages $\boldsymbol{v}$, as in Eq.~(\ref{eq:pretransform naive}), can be reduced by bringing pre-transform $\boldsymbol{T}$ into its systematic form $\boldsymbol{T}_\mathrm{sys}$, where $(\boldsymbol{T}_\mathrm{sys})_\mathcal{I}=\operatorname{RREF}(\boldsymbol{T}_\mathcal{I})$ is in \ac{RREF} and 
$(\boldsymbol{T}_\mathrm{sys})_\mathcal{F}=\boldsymbol{0}$.
Consequently, we find $\boldsymbol{u}_\mathcal{I}=\boldsymbol{v}_\mathcal{I}$.
Thus, the dynamic frozen bits at the einzelchild levels $f\in\mathcal{F} \setminus \mathbb{Z}_{i+1}$ can be computed as $u_f = \bigoplus_{h=i}^{f-1} u_h \cdot t_{h,f}$.

\begin{lemma}\label{lemma:M construction}
    Let $i<j<k$. If $\bar i \land j \land k = 0$ is fulfilled, then ${\mu_i(j,k) = (\bar i \land (j \lor k)) \lor (j \land k)} > k$.
\end{lemma}
\begin{proof}
    Let us split the bit positions in the support $\mathcal{S}_i$ of coset index $i$ as and the complementary set $\mathcal{S}_i^\mathrm{c}$.
    Subsequently, $l \in \mathcal S_i$ implies that ${\mu_i(j,k)_{(l)} = j_{(l)} \land k_{(l)}}$ and $l \in \mathcal{S}_i^\mathrm{c}$ implies that ${\mu_i(j,k)_{(l)} = j_{(l)} \lor k_{(l)}}$.
    Let the most significant bit index $l$ where $h_{(l)}>i_{(l)}$ be defined as 
    $l_i^*(h) = \max\left(\mathcal{S}_i^\mathrm{c} \cap \mathcal{S}_h\right)$.
    Consequently, if ${h > i}$, then $h_{(l)}=1$ for all $l \in \mathcal{S}_i \cap \mathbb{Z}_{l_i^*(h):n}$. 
    Thus, $l_i^*(k) > l_i^*(j)$ if $i < j < k$ as ${\bar i \land j \land k = 0}$. 
    We examine the most significant bit positions $\mathbb{Z}_{l_i^*(j):n}$.
    First, for $l \in \mathcal{S}_i \cap \mathbb{Z}_{l_i^*(j):n}$ we find $j_{(l)}=1$ as above and thus $\mu_i(j,k)_{(l)} = k_{(l)}$.
    Second, for ${l \in \mathcal{S}_i^\mathrm{c} \cap \mathbb{Z}_{l_i^*(j):n}}$ we find $j_{(l)}=0$ since ${l > l_i^*(j)}$ and thus $\mu_i(j,k)_{(l)} = k_{(l)}$.
    Finally, for $l = l_i^*(j)$ follows $\mu_i(j,k)_{(l)} > k_{(l)}$ and therefore $\mu_i(j,k) > k > j$.
\end{proof}

\begin{proposition}\label{proposition: Qiwmin tree}
    The message set $\mathcal{Q}_{i,\wmin}$ that forms the codewords of weight $\wmin$ of a universal polar coset $\mathcal P_i$ can be represented as a \ac{PDBT} with siblings levels ${\mathcal{L}_2 = \mathcal{K}_i}$.
\end{proposition}
\begin{proof}
    Let $\mathcal{J} \cup \{j\} \subseteq \mathcal{K}_i$ be a set of core rows obtained from $\mathcal{J}$ and $j$.
    From Lem.~\ref{lemma:M construction} and Eq.~(\ref{eq:add to Mset}) directly follows that ${\tilde{\mathcal M}_i(j,\mathcal J) \cap \mathbb Z_j = \emptyset}$, which implies with Eq.~(\ref{eq:Mset}) that 
    \begin{equation*}
        {\mathcal{M}_i(\mathcal{J}) \cap \mathbb{Z}_j} = {\mathcal{M}_i(\mathcal{J} \cup \{j\}) \cap \mathbb{Z}_j}.
    \end{equation*}
    In other words, all indices of the additional balancing rows $\tilde{\mathcal{M}}_i(j,\mathcal{J})$ for $\mathcal {M}_i(\mathcal{J} \cup \{j\})$ are greater than $j$.
    Correspondingly, by using Eq.~(\ref{eq:Ui set}) we find  for the message vectors 
    \begin{equation*}
        \boldsymbol{u}_{0:j}(i,\mathcal{J}) = \boldsymbol{u}_{0:j}(i,\mathcal{J} \cup \{j\}).
    \end{equation*}
    Further, $u_j(i,\mathcal{J}) < u_j(i,\mathcal{J} \cup \{j\})$, with which follows that $\mathcal{L}_2=\mathcal{K}_i$.
    We already saw that $\left|\mathcal Q_{i,\wmin}\right| = 2^{\left|\mathcal K_i\right|}$.
    Consequently, following Prop.~\ref{proposition:dichotomous binary tree}, $\mathcal{Q}_{i,\wmin}$ can be represented as a \ac{PDBT}.
\end{proof}


\begin{proposition}\label{proposition:update message}
    Let $\mathcal{J} \cup \{j\} \subseteq \mathcal{K}_i$ and $j > \max(\mathcal{J})$. Then a message ${\boldsymbol{u}(i,\mathcal{J})} \in \mathcal{Q}_{i,\wmin}$ can be computed as 
    \begin{equation}
        \begin{split}\label{eq:Ui set successive}
        \operatorname{supp}\left(\boldsymbol{u}(i,\mathcal{J} \cup \{j\})\right) &= \mathcal{U}_i(\mathcal{J} \cup \{j\})\\
        &= \left(\mathcal{U}_i(\mathcal{J}) \setxor \tilde{\mathcal{M}}_i(j,\mathcal{J}) \right) \cup \{j\},
        \end{split}
    \end{equation}       
    where the additional balancing rows are found as
    \begin{equation*}\label{eq:add to Mset successive}
        \tilde{\mathcal{M}}_i(j,\mathcal {J}) = \underset{{\substack{k \in \mathcal{U}_i(\mathcal{J}) \cap \mathbb{Z}_{i+1:j},\\\bar{i} \land j \land k = 0}}}{\bigsetxor} \left\{\mu_i(j,k)\right\}.  
    \end{equation*}
\end{proposition}
\begin{proof}
    Let ${x<y<z}$, then
    with $l_x^*(y) = \max\left(\mathcal{S}_x^\mathrm{c} \cap \mathcal{S}_y\right)$
    follows 
    $h_{(l)}=1$ for all $l \in \mathcal{S}_x \cap \mathbb{Z}_{l_x^*(y):n}$ and thus $l_x^*(z) \geq l_x^*(y)$.
    Consequently, for $j > \max\left(\mathcal J\right)$ follows $l_i^*(j) \geq l_i^*(\max(\mathcal J))$.
    Let $i < \min\{j,k\}$, then we find $l_i^*\left(\mu_i(j,k)\right) = l_i^*(\max\{j,k\})$.
    With Eq.~(\ref{eq:Mset}) and Eq.~(\ref{eq:add to Mset}) follows $l_i^*(j) \geq l_i^*(\max(\mathcal M_i(\mathcal J)))$. 
    Let ${\bar{i} \land j \land k = 0}$, then $l_i^*(j) \geq l_i^*(k)$ implies $j>k>i$.
    Thus, if $j > \max\left(\mathcal J\right)$, only rows $k \in \mathcal{U}_i(\mathcal{J}) \cap \mathbb{Z}_{i+1:j}$ have to be considered for the computation of $\tilde{\mathcal{M}}_i(j,\mathcal {J})$ with Eq.~(\ref{eq:add to Mset}).
    Subsequently, Eq.~(\ref{eq:Ui set successive}) follows from Eq.~(\ref{eq:Ui set}) and Eq.~(\ref{eq:Mset}).
\end{proof}

Following Prop.~\ref{proposition: Qiwmin tree} and Prop.~\ref{proposition:update message}, the messages $\boldsymbol{u} \in \mathcal{Q}_{i,\wmin}$ can be found without redundant operations from the tree.
Although both sets $\Qi$ and $\mathcal{Q}_{i,\wmin}$ can be represented as \acp{PDBT}, the message calculation differs.
For $\Qi$, the value of an einzelchild node is computed at the corresponding einzelchild level.
Thus, we only obtain a message $\boldsymbol{u} \in \Qi$ after we have followed a complete path through the tree.
In contrast, for $\mathcal{Q}_{i,\wmin}$, the values of the einzelchild nodes are determined at the sibling levels.
Hence, following Prop.~\ref{proposition:update message}, we directly find a message $\boldsymbol{u} \in \mathcal{Q}_{i,\wmin}$ if we update the set of core rows.


\subsection{Tree Intersection}
\begin{proposition}\label{proposition:tree intersection}
    The intersection tree $\mathcal{Z}$ of two \acp{DBT} $\mathcal{X}$, $\mathcal{Y}$ of height $N$ 
    with einzelchild levels $\mathcal{L}_{1,\mathcal{X}}$, $\mathcal{L}_{1,\mathcal{Y}}$,
    and sibling levels $\mathcal{L}_{2,\mathcal{X}}$, $\mathcal{L}_{2,\mathcal{Y}}$
    is again a \ac{DBT} with einzelchild levels
    \begin{equation*}
        \mathcal{L}_{1,\mathcal{Z}} = \left(\mathcal{L}_{1,\mathcal{X}} \cap \mathcal{L}_{1,\mathcal{Y}}\right) \cup \left(\mathcal{L}_{1,\mathcal{X}} \cap \mathcal{L}_{2,\mathcal{Y}}\right) \cup \left(\mathcal{L}_{2,\mathcal{X}} \cap \mathcal{L}_{1,\mathcal{Y}}\right)
    \end{equation*}
and sibling levels $\mathcal{L}_{2,\mathcal{Z}} = \mathcal{L}_{2,\mathcal{X}} \cap \mathcal{L}_{2,\mathcal{Y}}$.
\end{proposition}
\begin{proof}
    If the root note of $\mathcal{X}$ and $\mathcal{Y}$ is equal, the intersection tree $\mathcal{Z}$ has the same root node.
    Otherwise, $\mathcal{Z}$ is empty.
    From the root node onward, $\mathcal{Z}$ is found successively level by level.
    A node in $\mathcal{Z}$ has a left and/or right child node if and only if both $\mathcal{X}$ and $\mathcal{Y}$ contain the corresponding node. 
    As $\mathcal{X}$ and $\mathcal{Y}$ are both dichotomous, there are four cases of levels:
    \begin{enumerate}
        \item $l \in \mathcal{L}_{1,\mathcal{X}} \cap \mathcal{L}_{1,\mathcal{Y}}$:
        A node in $\mathcal{Z}$ at level $l-1$ has the same child node as the corresponding nodes in $\mathcal{X}$ and in $\mathcal{Y}$ if their child nodes coincide. Otherwise, it is a leaf node.    
        \item $l \in \mathcal{L}_{1,\mathcal{X}} \cap \mathcal{L}_{2,\mathcal{Y}}$:
        A node in $\mathcal{Z}$ at level $l-1$ has the same child node as the corresponding node in $\mathcal{X}$.
        \item $l \in \mathcal{L}_{2,\mathcal{X}} \cap \mathcal{L}_{1,\mathcal{Y}}$:
        A node in $\mathcal{Z}$ at level $l-1$ has the same child node as the corresponding node in $\mathcal{Y}$.
        \item $l \in \mathcal{L}_{2,\mathcal{X}} \cap \mathcal{L}_{2,\mathcal{Y}}$:
        All nodes in $\mathcal{Z}$ are sibling nodes.
    \end{enumerate}
    Subsequently, cases 1) to 3) correspond to the einzelchild levels $\mathcal{L}_{1,\mathcal{Z}}$ of $\mathcal{Z}$ and case 4) to the sibling levels $\mathcal{L}_{2,\mathcal{Z}}$.
    Therefore, $\mathcal{Z}$ is dichotomous.
\end{proof}


From Prop.~\ref{proposition:tree intersection} follows that the intersection tree of the \acp{PDBT} corresponding to $\Qi$ and $\mathcal{Q}_{i,\wmin}$ is a \ac{DBT} with sibling levels $\mathcal{L}_2 = \mathcal{I} \cap \mathcal{K}_i$. 
Subsequently, to find a message $\boldsymbol{u} \in \Qiwmin$, 
the bits at levels $\mathcal{I} \cap \mathcal{K}_i$ can be chosen freely.
The bits at levels $\mathcal{I} \cap \mathcal{K}_i^\mathrm{c}$ are determined by the pre-transformation.
For ``1'' bits at these levels $\mathcal{K}_i$, $\boldsymbol{u}$ is updated as in Prop.~\ref{proposition:update message}.
The nodes of levels $\mathcal{I} \cap \mathcal{K}_i^\mathrm{c}$ are
predetermined from the levels $\mathcal{K}_i$ and the bits at levels $\mathcal{I} \cap \mathcal{K}_i^\mathrm{c}$ can be chosen accordingly.
For bits $\mathcal{F} \cap \mathcal{K}_i^\mathrm{c}$ both trees of  $\Qi$ and $\mathcal{Q}_{i,\wmin}$ have einzelchild levels.
Consequently, the current message $\boldsymbol{u}$ and the pre-transformation have to match.
If not, then we found a leaf node of the intersection tree and the message path does not form a $\wmin$-weight codeword of the code.

Conversely, for level $f_i^*(\mathcal{I}) = \max\left(\{i\} \cup \left(\mathcal{F} \cap \mathcal{K}_i^\mathrm{c}\right)\right)$, the subsequent sub-tree is a \ac{PDBT} with sibling levels $\mathcal{K}_i^\circ = \mathcal{K}_i \setminus \mathbb{Z}_{f_i^*(\mathcal{I})}$ and 
we can simply write the enumeration as
\begin{equation}\label{eq:Awmin subtree simplification}
    \left|\Qiwmin\right| = \left|\mathcal{Q}_{i,\wmin}(\mathcal{I} \setminus \mathcal{K}_i^\circ,\boldsymbol{T})\right| \cdot 2^{\left|\mathcal{I} \cap \mathcal{K}_i^\circ\right|}.
\end{equation}
Following this, Alg.~\ref{alg:error_coeff} recursively traverses the intersection tree in \emph{reverse pre-order} and counts the $\wmin$-weight codewords.


\begin{algorithm}[tbh]
    \small%
    \SetAlgoLined\LinesNumbered
    \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
    \Input{Information set $\mathcal I$, pre-transformation matrix $\boldsymbol T$}
    \Output{Number of $\wmin$-weight codewords $A_{\wmin}$}
    $\boldsymbol{T}_\mathcal{I} \gets \operatorname{RREF}(\boldsymbol{T}_\mathcal{I}),\;\boldsymbol{T}_\mathcal{F} \gets \boldsymbol{0}$\;
    \Return $\sum_{i \in \mathcal I_{\wmin}} \operatorname{enum\_subtree}(i,i,\boldsymbol{0},\mathcal {I},\boldsymbol{T}) \cdot 2^{|\mathcal{I} \cap \mathcal{K}_i^\circ|}$\;
    \algrule[.5pt]
    \Fn{$\operatorname{enum\_subtree}(i,j,\boldsymbol u,\mathcal {I},\boldsymbol{T})$}{
    $A_{i,\wmin} \gets 0$\;
    	$\boldsymbol{u} \gets \operatorname{update\_message}(i,j,\operatorname{copy}(\boldsymbol{u}))$\;
        \For{$k \gets j+1$ \KwTo $f_i^*(\mathcal{I})$}{
            \uIf{$k \in \mathcal{I} \cap \mathcal{K}_i$}{
                $A_{i,\wmin} \gets A_{i,\wmin} + \operatorname{enum\_subtree}(i,k,\boldsymbol u,\mathcal {I},\boldsymbol{T})$\;
            }
            \Else{
                $d \gets \bigoplus_{h=i}^{k-1} u_h \cdot t_{h,k}$\;\vspace{0.025cm}
                \uIf{$k \in \mathcal K_i^\mathrm{c}$}{
                        \lIf{$d \neq u_k$}{\Return $A_{i,\wmin}$}
                    }
                \ElseIf{$d = 1$}{
                $\boldsymbol{u} \gets \operatorname{update\_message}(i,k,\boldsymbol{u})$\;
                }
            }
        }
        \Return $A_{i,\wmin}$ + 1\;
    }
    \algrule[.5pt]
    \Fn{$\operatorname{update\_message}(i,j,\boldsymbol{u})$}{
        \For{$k \gets i+1$ \KwTo $j-1$\label{algline:i+1 to j-1}}{
            \If{$u_k = 1$ \rm{\textbf{and}} $\bar i \land j \land k = 0$}{
                $u_{\mu_i(j,k)} \gets u_{\mu_i(j,k)} \oplus 1$\;
            }
        }
        $u_j \gets 1$\;
        \Return $\boldsymbol{u}$\;
    }
	\caption{\footnotesize
	$\operatorname{error\_coefficient}(\mathcal I,\boldsymbol T)$
    }
    \label{alg:error_coeff}
\end{algorithm}


\begin{example}
    \normalfont Consider the case $N=16$ and $\wmin=4$. We regard the coset $\mathcal P_{i=10}$. Using Eq.~(\ref{eq:ki}), we find $\mathcal{K}_{i=10}=\{11,12,14\}$ and $\mathcal{K}^\mathrm{c}_{i=10}=\{13,15\}$. Hence, there are $2^{|\mathcal{K}_{i=10}|}=8$ weight-4 codewords in this coset. The corresponding \ac{PDBT} of the messages generating these $\wmin$-weight codewords is shown in Fig.~\ref{subfig:tree_universal}.
    Now consider the rate-profile ${\mathcal{I}=\{10,11,14,15\}}$. The coset $\mathcal{Q}_{i=10}(\mathcal{I})$ forms the \ac{PDBT} depicted in Fig.~\ref{subfig:tree_rate_profile}. The intersection of both trees is $\mathcal{Q}_{i=10,\wmin=4}(\mathcal{I})$ and highlighted; it contains 4 weight-4 codewords. In this case, the leaf nodes of the intersection tree are at the level $N-1$.
\end{example}

==> tikzlibrarydsp.code.tex <==

\usetikzlibrary{arrows, calc, positioning, decorations.markings}


\newcommand{\dsplinewidth}{0.25mm}           %
\newcommand{\dspblocklinewidth}{0.3mm}       %
\newcommand{\dspoperatordiameter}{4mm}       %
\newcommand{\dspoperatorlabelspacing}{2mm}   %
\newcommand{\dspnoderadius}{1mm}             %
\newcommand{\dspsquareblocksize}{8mm}        %
\newcommand{\dspfilterwidth}{14mm}           %


\pgfarrowsdeclare{dsparrow}{dsparrow}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt} %
	\pgfsetmiterjoin	 %
	\pgfsetbuttcap		 %
	\pgfpathmoveto{\pgfpoint{-4\arrowsize}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{4\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{-4\arrowsize}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}

\pgfarrowsdeclare{dsparrowmid}{dsparrowmid}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfarrowsleftextend{-4\arrowsize}
	\pgfarrowsrightextend{4\arrowsize}
}
{
	\arrowsize=0.25pt
	\advance\arrowsize by .5\pgflinewidth
	\pgfsetdash{}{0pt}
	\pgfsetmiterjoin
	\pgfsetbuttcap
	\pgfpathmoveto{\pgfpoint{0}{2.5\arrowsize}}
	\pgfpathlineto{\pgfpoint{8\arrowsize}{0pt}}
	\pgfpathlineto{\pgfpoint{0}{-2.5\arrowsize}}
	\pgfpathclose
	\pgfusepathqfill
}


\makeatletter

\pgfkeys{/tikz/dsp/label/.initial=above}

\long\def\dspdeclareoperator#1#2{
	\pgfdeclareshape{#1}
	{
		\savedanchor\centerpoint{\pgfpointorigin}
		\savedmacro\label{\def\label{\pgfkeysvalueof{/tikz/dsp/label}}}
	  \saveddimen\radius
	  {
		  \pgfmathsetlength\pgf@xa{\pgfshapeminwidth}
		  \pgfmathsetlength\pgf@ya{\pgfshapeminheight}
	    \ifdim\pgf@xa>\pgf@ya
	      \pgf@x=.5\pgf@xa
	    \else
	      \pgf@x=.5\pgf@ya
	    \fi
	  }
	  
	  %
	  \inheritanchor[from={circle}]{center}
	  \inheritanchor[from={circle}]{mid}
	  \inheritanchor[from={circle}]{base}
	  \inheritanchor[from={circle}]{north}
	  \inheritanchor[from={circle}]{south}
	  \inheritanchor[from={circle}]{west}
	  \inheritanchor[from={circle}]{east}
	  \inheritanchor[from={circle}]{mid west}
	  \inheritanchor[from={circle}]{mid east}
	  \inheritanchor[from={circle}]{base west}
	  \inheritanchor[from={circle}]{base east}
	  \inheritanchor[from={circle}]{north west}
	  \inheritanchor[from={circle}]{south west}
	  \inheritanchor[from={circle}]{north east}
	  \inheritanchor[from={circle}]{south east}
	  \inheritanchorborder[from={circle}]
	  
	  %
	  \backgroundpath
	  {
	    %
	    \pgfpathcircle{\centerpoint}{\radius}
	    
	    %
	    %
	    #2
	  }
	
	  \anchor{text}
	  {
			\centerpoint
	    \def\templabelabove{above}
	    \def\templabelbelow{below}
	    \def\templabelleft{left}
	    \def\templabelright{right}
	    \pgfutil@tempdima=\dspoperatorlabelspacing
	    %
	    \ifx\label\templabelabove
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by \radius
				\advance\pgf@y by \pgfutil@tempdima
	    \fi
	    %
	    \ifx\label\templabelbelow
				\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
				\advance\pgf@y by -\radius
				\advance\pgf@y by -\pgfutil@tempdima
				\advance\pgf@y by -\ht\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelleft
				\advance\pgf@x by -\radius
				\advance\pgf@x by -\pgfutil@tempdima
				\advance\pgf@x by -\wd\pgfnodeparttextbox
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	    %
	    \ifx\label\templabelright
				\advance\pgf@x by \radius
				\advance\pgf@x by \pgfutil@tempdima
				\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
				\advance\pgf@y by +0.5\dp\pgfnodeparttextbox
	    \fi
	  }
	}
}

\dspdeclareoperator{dspshapecircle}{\pgfusepathqstroke}

\dspdeclareoperator{dspshapecirclefull}{\pgfusepathqfillstroke}

\dspdeclareoperator{dspshapeadder}{
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.55\pgfutil@tempdima
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{0pt}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{0pt}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{0pt}}}
	
	\pgfusepathqstroke
}

\dspdeclareoperator{dspshapemixer}{
	\pgfutil@tempdima=\radius
	\pgfutil@tempdima=0.707106781\pgfutil@tempdima
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{-\pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{ \pgfutil@tempdima}}}
	
	\pgfmoveto{\pgfpointadd{\centerpoint}{\pgfpoint{-\pgfutil@tempdima}{ \pgfutil@tempdima}}}
	\pgflineto{\pgfpointadd{\centerpoint}{\pgfpoint{ \pgfutil@tempdima}{-\pgfutil@tempdima}}}
	
	\pgfusepathqstroke
}

\makeatother


\tikzset{dspadder/.style={shape=dspshapeadder,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmultiplier/.style={shape=dspshapecircle,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}
\tikzset{dspmixer/.style={shape=dspshapemixer,line cap=rect,line join=rect,
	line width=\dspblocklinewidth,minimum size=\dspoperatordiameter}}

\tikzset{dspnodeopen/.style={shape=dspshapecircle,line width=\dsplinewidth,minimum size=\dspnoderadius}}
\tikzset{dspnodefull/.style={shape=dspshapecirclefull,line width=\dsplinewidth,fill,minimum size=\dspnoderadius}}

\tikzset{dspsquare/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum size=\dspsquareblocksize}}
\tikzset{dspfilter/.style={shape=rectangle,draw,align=center,text depth=0.3em,text height=1em,inner sep=0pt,
	line cap=round,line join=round,line width=\dsplinewidth,minimum height=\dspsquareblocksize,minimum width=\dspfilterwidth}}


\tikzset{dspline/.style={line width=\dsplinewidth},line cap=round,line join=round}
\tikzset{dspconn/.style={->,>=dsparrow,line width=\dsplinewidth},line cap=round,line join=round}%
\tikzset{dspflow/.style={line width=\dsplinewidth,line cap=round,line join=round,
  decoration={markings,mark=at position 0.5 with {\arrow{dsparrowmid}}},postaction={decorate}}}


\newcommand{\downsamplertext}[1]{\raisebox{0.1em}{$\big\downarrow$}#1}
\newcommand{\upsamplertext}[1]{\raisebox{0.1em}{$\big\uparrow$}#1}


==> tikzlibrarymux.code.tex <==
\tikzset{every mux2 node/.style={draw,minimum width=0.6cm,minimum height=2cm,inner sep=1mm,outer sep=0pt}}
\tikzset{every mux3 node/.style={draw,minimum width=0.6cm,minimum height=3cm,inner sep=1mm,outer sep=0pt}}
\tikzset{every mux4 node/.style={draw,minimum width=0.6cm,minimum height=4cm,inner sep=1mm,outer sep=0pt}}
\tikzset{every mux5 node/.style={draw,minimum width=0.6cm,minimum height=4.8cm,inner sep=1mm,outer sep=0pt}}

\pgfdeclareshape{mux2}{

  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  \inheritanchorborder[from=rectangle]
  
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{
    \pgf@process{\northeast}%
    \pgf@y=.25\pgf@y%
  }
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  \anchor{in0}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.5\pgf@y%
  }
  \anchor{in1}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.5\pgf@y%
  }
  \anchor{sel}{
    \pgf@process{\northeast}%
    \pgf@x=0pt%
    \pgf@y=-0.7\pgf@y%
  }

  \anchor{out}{
    \pgf@process{\northeast}%
    \pgf@y=0pt%
  }

  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \let\pgf@xnw=\pgf@xa
    \let\pgf@ynw=\pgf@yb
    \let\pgf@xsw=\pgf@xa
    \let\pgf@ysw=\pgf@ya
    \let\pgf@xse=\pgf@xb
    \pgf@yc=-\pgf@yb
    \advance\pgf@yc by \pgfshapeminwidth
    \let\pgf@yse=\pgf@yc
    \let\pgf@xne=\pgf@xb
    \pgf@xc=\pgf@yb
    \advance\pgf@xc by -\pgfshapeminwidth
    \let\pgf@yne=\pgf@xc
    \pgfpathmoveto{\pgfpoint{\pgf@xnw}{\pgf@ynw}}
    \pgfpathlineto{\pgfpoint{\pgf@xsw}{\pgf@ysw}}
    \pgfpathlineto{\pgfpoint{\pgf@xse}{\pgf@yse}}
    \pgfpathlineto{\pgfpoint{\pgf@xne}{\pgf@yne}}
    \pgfpathclose
  }
}

\pgfdeclareshape{mux3}{

  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  \inheritanchorborder[from=rectangle]
  
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{
    \pgf@process{\northeast}%
    \pgf@y=.25\pgf@y%
  }
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  \anchor{in0}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.5\pgf@y%
  }
  \anchor{in1}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=0pt%
  }
  \anchor{in2}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.5\pgf@y%
  }
  \anchor{sel}{
    \pgf@process{\northeast}%
    \pgf@x=0pt%
    \pgf@y=-0.75\pgf@y%
  }

  \anchor{out}{
    \pgf@process{\northeast}%
    \pgf@y=0pt%
  }

  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \let\pgf@xnw=\pgf@xa
    \let\pgf@ynw=\pgf@yb
    \let\pgf@xsw=\pgf@xa
    \let\pgf@ysw=\pgf@ya
    \let\pgf@xse=\pgf@xb
    \pgf@yc=-\pgf@yb
    \advance\pgf@yc by \pgfshapeminwidth
    \let\pgf@yse=\pgf@yc
    \let\pgf@xne=\pgf@xb
    \pgf@xc=\pgf@yb
    \advance\pgf@xc by -\pgfshapeminwidth
    \let\pgf@yne=\pgf@xc
    \pgfpathmoveto{\pgfpoint{\pgf@xnw}{\pgf@ynw}}
    \pgfpathlineto{\pgfpoint{\pgf@xsw}{\pgf@ysw}}
    \pgfpathlineto{\pgfpoint{\pgf@xse}{\pgf@yse}}
    \pgfpathlineto{\pgfpoint{\pgf@xne}{\pgf@yne}}
    \pgfpathclose
  }
}

\pgfdeclareshape{mux4}{

  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  \inheritanchorborder[from=rectangle]
  
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{
    \pgf@process{\northeast}%
    \pgf@y=.25\pgf@y%
  }
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  \anchor{in0}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.6\pgf@y%
  }
  \anchor{in1}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=0.2\pgf@y%
  }
  \anchor{in2}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.2\pgf@y%
  }
  \anchor{in3}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.6\pgf@y%
  }
  \anchor{sel}{
    \pgf@process{\northeast}%
    \pgf@x=0pt%
    \pgf@y=-0.85\pgf@y%
  }

  \anchor{out}{
    \pgf@process{\northeast}%
    \pgf@y=0pt%
  }

  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \let\pgf@xnw=\pgf@xa
    \let\pgf@ynw=\pgf@yb
    \let\pgf@xsw=\pgf@xa
    \let\pgf@ysw=\pgf@ya
    \let\pgf@xse=\pgf@xb
    \pgf@yc=-\pgf@yb
    \advance\pgf@yc by \pgfshapeminwidth
    \let\pgf@yse=\pgf@yc
    \let\pgf@xne=\pgf@xb
    \pgf@xc=\pgf@yb
    \advance\pgf@xc by -\pgfshapeminwidth
    \let\pgf@yne=\pgf@xc
    \pgfpathmoveto{\pgfpoint{\pgf@xnw}{\pgf@ynw}}
    \pgfpathlineto{\pgfpoint{\pgf@xsw}{\pgf@ysw}}
    \pgfpathlineto{\pgfpoint{\pgf@xse}{\pgf@yse}}
    \pgfpathlineto{\pgfpoint{\pgf@xne}{\pgf@yne}}
    \pgfpathclose
  }
}

\pgfdeclareshape{mux5}{

  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  \inheritanchorborder[from=rectangle]
  
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{
    \pgf@process{\northeast}%
    \pgf@y=.25\pgf@y%
  }
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  \anchor{in0}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.7\pgf@y%
  }
  \anchor{in1}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=0.35\pgf@y%
  }
  \anchor{in2}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=0\pgf@y%
  }
  \anchor{in3}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.35\pgf@y%
  }
  \anchor{in4}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.7\pgf@y%
  }
  \anchor{sel}{
    \pgf@process{\northeast}%
    \pgf@x=0pt%
    \pgf@y=-0.75\pgf@y%
  }

  \anchor{out}{
    \pgf@process{\northeast}%
    \pgf@y=0pt%
  }

  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \let\pgf@xnw=\pgf@xa
    \let\pgf@ynw=\pgf@yb
    \let\pgf@xsw=\pgf@xa
    \let\pgf@ysw=\pgf@ya
    \let\pgf@xse=\pgf@xb
    \pgf@yc=-\pgf@yb
    \advance\pgf@yc by \pgfshapeminwidth
    \let\pgf@yse=\pgf@yc
    \let\pgf@xne=\pgf@xb
    \pgf@xc=\pgf@yb
    \advance\pgf@xc by -\pgfshapeminwidth
    \let\pgf@yne=\pgf@xc
    \pgfpathmoveto{\pgfpoint{\pgf@xnw}{\pgf@ynw}}
    \pgfpathlineto{\pgfpoint{\pgf@xsw}{\pgf@ysw}}
    \pgfpathlineto{\pgfpoint{\pgf@xse}{\pgf@yse}}
    \pgfpathlineto{\pgfpoint{\pgf@xne}{\pgf@yne}}
    \pgfpathclose
  }
}

